ProgressiveMotionSeg: Mutually Reinforced Framework for Event-Based Motion Segmentation

Dynamic Vision Sensor (DVS) can asynchronously output the events reflecting apparent motion of objects with microsecond resolution, and shows great application potential in monitoring and other fields. However, the output event stream of existing DVS inevitably contains background activity noise (BA noise) due to dark current and junction leakage current, which will affect the temporal correlation of objects, resulting in deteriorated motion estimation performance. Particularly, the existing filter-based denoising methods cannot be directly applied to suppress the noise in event stream, since there is no spatial correlation. To address this issue, this paper presents a novel progressive framework, in which a Motion Estimation (ME) module and an Event Denoising (ED) module are jointly optimized in a mutually reinforced manner. Specifically, based on the maximum sharpness criterion, ME module divides the input event into several segments by adaptive clustering in a motion compensating warp field, and captures the temporal correlation of event stream according to the clustered motion parameters. Taking temporal correlation as guidance, ED module calculates the confidence that each event belongs to real activity events, and transmits it to ME module to update energy function of motion segmentation for noise suppression. The two steps are iteratively updated until stable motion segmentation results are obtained. Extensive experimental results on both synthetic and real datasets demonstrate the superiority of our proposed approaches against the State-Of-The-Art (SOTA) methods.

==> sections/experiment_jz.tex <==
The intrinsic parameter of simulated camera is also specified like the one of DAVIS240 \cite{brandli2014240} but without distortion. Specifically, the resolution is 240x180, $f_x=f_y=200$, $c_x=120,c_y=90$. All further experiments inherit this setting.

Testing results in the simulated environments are shown qualitatively in Fig.\ref{fig:env}. Four scenes have different textures and occlusion settings (0 to 3 occluded areas) with only 3 moving objects. The noise level is 05 for all these scenes.

In general, it can be seen that our method outperforms other existing methods in the task of motion segmentation. Specifically, compared to the result of direct segmentation, our method filters out outliers and as a result improves the segmentation consistency inside different areas, as is shown in scene 2 where isolated events are removed and points that lie in other areas are also fixed to become the right ones.


It's worth noting that in Scene 1 and Scene 3, the structure is not apparent while our method successfully recovers the right texture. From the perspective of motion segmentation, because the texture is very dense, the generated events are also very dense. It's difficult for simple motion segmentation to eliminate the influence of other motions due to the effect of the normalizing factor, so that the dense segmentation results are close to each other, and the estimated motion parameters are offset from the real parameters. However, our method successfully recovered the real motion because the influence from other motions is quickly reduced.

Compared to the result of first denoising and then segmenting motions, our method does not damage the structural information of the event stream, and thus has better segmentation performance. Specifically, from scene 2 it can be seen that the denoising methods do remove a large part of isolated event points, but at the same time it also filters out a large number of useful event points, which greatly reduces the discrimination of different events. In this manner, Knoise shows no difference from Ynoise in terms of noise model because of the excessive damage to the structural information.
\begin{figure*}
    \begin{center}
        \includegraphics[width=1.0\textwidth]{Images/Visio-Figure_RealScene.pdf}
    \end{center}
    \caption{Segmentation results for real-world sequences slider\_depth \cite{rebecq2016emvs} and what\_is\_the\_background \cite{mitrokhinevent}. Red boxes highlight segmentation difference between direct segmentation and our method.}
    \label{fig:real}
\end{figure*}


Quantitative results are shown in Fig.\ref{fig:roc} as ROC curves for our method and isolated points in the ROC plane for other methods. The reason is that different configurations for those methods don't have much influence on the performance so we only report the best possible result.


In order to quantify the robustness of our method under different noise levels, we use different contrast thresholds to generate different event streams in scene 2 and test the denoising effect. We also provide ROC curves under different noise levels as shown in Fig.\ref{fig:robustness_to_noise}. It should be noted that when the noise level is higher than 15, the contrast threshold is already lower than 3$\sigma$.

It can be seen from the motion compensation graph (b) to (d) that our method can still filter out the noise while providing better motion-compensated event images under different noise levels. However, as the noise level continues to increase, the number of misclassified events gradually increases. This is in line with our intuition. It can be seen from the ROC curves (a) that as the noise level increases, the performance of segmentation gradually decreases, but when the noise level is lower than 20, the difference between them is not obvious. At the same time, our curve is very close to the ideal point (0,1), which further illustrates the effectiveness of our method.

As is shown by the result of direct motion segmentation without denoising, noise has great impact on the segmentation result. For those events that should not have appeared, the segmentation method will still forcefully determine which motion group they belong to. As a result, the segmentation performance of normal events will also be affected. As is shown at the lower right area of compensated images, the aliasing effect appears.

As denoising progresses, it can be seen that those discrete points in space are gradually eliminated, which by itself confirms the assumption that the segmentation results of these points are unstable. In the same area, the segmentation results with wrong motion information are gradually corrected due to the elimination of noise. This process embodies the mutual promotion characteristics of our method, showing the superiority of our framework.

\begin{table}[]
\caption{Comparison results with different methods on EED dataset (in $\%$). FMD, LV, WIB, OC and MO represnet the fast moving drone, lighting variations, what is background, occluded sequence, multiple objects scene, respectively. }
\small
\begin{tabular}{c|ccccc}
\hline
EED Sequence Name                    & FMD                                    & LV                                    & WIB                                   & OS                                    & MO                                    \\ \hline
Knoise+EBMS                          &                                       &                                       &                                       &                                       &                                       \\
Ynoise+EBMS                          &                                       &                                       &                                       &                                       &                                       \\
EBMS                                 & 27.17                                 & 30.95                                 & 68.43                                 & 69.66                                 & 41.63                                 \\ \hline
{\color[HTML]{FF0000} \textbf{Ours}} & {\color[HTML]{FF0000} \textbf{53.92}} & {\color[HTML]{FF0000} \textbf{48.33}} & {\color[HTML]{FF0000} \textbf{93.33}} & {\color[HTML]{FF0000} \textbf{83.23}} & {\color[HTML]{FF0000} \textbf{51.11}} \\ \hline
\end{tabular}
\end{table}
\subsection{Comparisons on Real-word DVS Data}
The Extreme Event Dataset (EED) \cite{mitrokhinevent} is an event segmentation dataset which contains very challenging sequences for conventional cameras, i.e. ultra low light and ultra fast motion, which contain a large amount of noise. We compare our results with the SOTA motion segmentation method \cite{stoffregen2019event}. In their work an object is successfully detected if the estimated bounding box overlaps at least 50\% with the hand-labeled one and for most sequences their success rates are no no less than 90\%. But that cannot demonstrate the superiority of our proposed method, so we instead calculate the percentage of correctly segmented events as those lying inside the hand-labeled bounding boxes.

\textbf{The Effect of Denoising in Motion Segmentation\quad}Current denoising methods do not contribute to motion segmentation but instead leading to a decrease in performance. The reason is that: existing denoising methods are based on the spatio-temporal correlation feature of event stream. In theory, this can indeed be used to identify the noise, but event points that do not have spatio-temporal correlation may also contain motion information, and the impact of denoising is dependent on the pixel location. Therefore, the result of denoising in the spatio-temporal domain based on the globally consistent spatio-temporal correlation will lead to the destruction of the inconsistent motion information, i.e., more information is removed where motion is obvious, which leads to the decline of the motion segmentation performance, as is shown in Fig.\ref{fig:env} and \ref{fig:real}.

Specifically, the calculation of spatio-temporal correlation must be based on known events, and a large number of events appear in the motion area. This method itself has a tendency to sample event points generated by real motion more often. The second is that motion does not necessarily include only spatial translational motion that is uniform in time. Some motions, such as rotational motion, have different spatio-temporal correlation properties at different distances from the center of the rotation. The third is that even if the motion is uniform in space, under the influence of noise, there may still be intermittently spatial inconsistent areas. This, supplemented by its own biased sampling tendency, brings poor motion segmentation results. Therefore, in order to improve the effect of motion estimation, the design of the denoising module must be combined with the task of motion estimation itself to get better results.

To show that our denoising module can really improve the performance of motion segmentation, we evaluate our method both on simulation environment extensively and real-world sequences qualitatively. For the simulation environment, we use the ESIM \cite{rebecq2018esim} simulator, which is state-of-the-art and can adjust noise level as the standard deviation of contrast threshold to evaluate the robustness of our method. For real-world event sequences, since there's currently no existing public dataset for this purpose, we only show qualitative results. For all the sequences, we take up to 20000 events one time for motion segmentation, which lasts for 30-100ms in time for consistent illumination and motion.

We also provide motion-compensated event images after being denoised for qualitative comparison. Instead of segmented based on the probability of event assignment, we only overlay images with opacity set to respective weight to show that the weights can also be viewed as a better representation of event segmentation.

Throughout the experiments, we show that our method has the best segmentation performance due to the correct design of both the framework and the denoise module: \textit{(i)} the fact that the ED module and ME module works in a mutually reinforced manner enables them to correct each other, leading to better results on both, \textit{(ii)} the denoise module preserves more motion information because its relation with motion is explicitly modeled, which improves the performance of motion segmentation, \textit{(iii)} the good noise model enables our method to operate on varying noise levels, adding to the robustness of our method.


\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{Images/diff_noise.pdf}
    \caption{Segmentation results under different noise levels (b)-(d) and ROC curve (a).}
    \label{fig:robustness_to_noise}
\end{figure}


% \textbf{Robustness of Segmentation under Varying Noise Levels\quad}In order to quantify the robustness of our method under different noise levels, we use different contrast thresholds to generate different event streams in scene 2 and test the denoising effect. We also provide ROC curves under different noise levels as shown in Fig.\ref{fig:robustness_to_noise}. It should be noted that when the noise level is higher than 15, the contrast threshold is already lower than 3$\sigma$.

% It can be seen from the motion compensation graph (b) to (d) that our method can still filter out the noise while providing better motion-compensated event images under different noise levels. However, as the noise level continues to increase, the number of misclassified events gradually increases. This is in line with our intuition. It can be seen from the ROC curves (a) that as the noise level increases, the performance of segmentation gradually decreases, but when the noise level is lower than 20, the difference between them is not obvious. At the same time, our curve is very close to the ideal point (0,1), which further illustrates the effectiveness of our method.

% As is shown by the result of direct motion segmentation without denoising, noise has great impact on the segmentation result. For those events that should not have appeared, the segmentation method will still forcefully determine which motion group they belong to. As a result, the segmentation performance of normal events will also be affected. As is shown at the lower right area of compensated images, the aliasing effect appears.

% As denoising progresses, it can be seen that those discrete points in space are gradually eliminated, which by itself confirms the assumption that the segmentation results of these points are unstable. In the same area, the segmentation results with wrong motion information are gradually corrected due to the elimination of noise. This process embodies the mutual promotion characteristics of our method, showing the superiority of our framework.

==> sections/proposed_method.tex <==
\section{Proposed Method}
\subsection{Overview of Progressive Framework}

Given a package of noisy events, our goal is to segment real activity events into independently-moving objects while suppressing the noise influence. To this end, we propose an effective progressive learning framework by optimizing the motion estimation and event denoising in a mutually reinforced manner. As is shown in Fig.\ref{fig:cycle}, our proposed progressive framework consists of two modules: the Motion Estimation (ME) module and the Event Denoising (ED) module.

Taking event stream as input, the ME module first conducts adaptive clustering by warping the events to a reference time and maximizing their alignment. Based on the clustering results, we can estimate the motion parameters. After that, temporal correlation of event stream is calculated by utilizing the estimated motion parameters and transmitted to ED module to guide the event denoising. Taking the temporal correlation map as input, ED module first maps the correlation value to event confidence belonging to [0,1]. The confidence value represents the probability of event belonging to noise, and the greater the confidence value, the greater the possibility of being real activity event. Then, the confidence value is multiplied to the event, which is transmitted to ME module to update the motion estimation. Each of the preceding two processes benefits from the gradual improvement results in the other. We progressively perform the two processes until obtaining stable results.

\subsection{Motion Estimation Module}
The output of DVS, or event stream takes the form of spatio-temporal pointcloud, i.e. $E=\{e_k=(\bm{x}_k,t_k,b_k)|k=1,2...N_e\}$, where each event $e_k$ represents a change in logarithmic intensity at pixel $\bm{x}_k$ and time $t_k$ % 要不要说明下噪声很大
\begin{equation}
    \Delta L(\bm{x}_k,t_k)=L(\bm{x}_k,t_k)-L(\bm{x}_k, t_k-\Delta t_k)=b_k C,
\end{equation}
where $L(\bm{x},t)=logI(\bm{x},t)$, $C$ is contrast threshold and $b_k$ is the polarity representing the direction of intensity change. We can accumulate events along respective warping field to a reference time to build an Image of Warped Events (IWE) as
\begin{equation}
    \mathrm{IWE}(\bm{x})=\sum_{k=1}^{N_e}w_k\delta(\bm{x}-\bm{x}_{k}'),
\end{equation}
where $w_k$ is the possible weight and $\bm{x}_k'=\bm{\mathrm{W}}(\bm{x}_k,t_k;\bm{\theta})$ is the warped event location by a warping parameter $\bm{\theta}$
\begin{equation}
    e_k=(\bm{x}_k,t_k,b_k)\mapsto e_k'=(\bm{x}_k',t_{ref},b_k).
\end{equation}
Then the sharpness of the warped image can be used to measure the goodness of fit between the warping field and the event data\cite{}.

For event-based motion segmentation, event clustering is performed in the warping field space. In \cite{} this is done by substituting the weights with event probability and optimizing in each motion cluster. In this work we take a step further in that we additionally assigns a confidence for each combination of events and clusters which will be further explained in our ED module.

The Motion Estimation module tries to find the solution to this maximization problem as
\begin{align}
    % \mathrm{maximize} \underset{(\bm{\theta},\bm{\mathrm{P}},\bm{\mathrm{C}})}{\arg\max}\sum_{j=1}^{N_l}Sharpness(I_j)\\
    \max_{(\bm{\theta},\bm{\mathrm{P}},\bm{\mathrm{C}})}\quad &\sum_{j=1}^{N_l}\mathrm{Sharpness}(I_j)\\
    \mathrm{s.t.} \quad & I_j(\bm{x}) = \sum_{k=1}^{N_e}c_{kj}p_{kj}\delta(\bm{x}-\bm{x}_{kj}')\\
    &\sum_{j=1}^{N_l}p_{kj} = 1,\quad p_{kj} \geq 0 \\
    &c_{kj} \in [0,1]
\end{align}
where $N_l$ is the number of clusters, $\bm{x}_{kj}'$ is the warped location of the kth event  $e_k$, $p_{kj}$ and $c_{kj}$ are event assignment probability and event confidence respectively. To explain our sharpness metric, we need to first define our events correlation image.

\textbf{Warped Event Image As Event Correlation Representation \quad} Based on the brightness constancy constraint\cite{}, we have that along the pixel trajectory
\begin{equation}
    \frac{\partial L}{\partial t} = -\nabla L \cdot v,
\end{equation}
and from the DVS working principle, if $\Delta t$ is small enough, we have
\begin{equation}
    \frac{\partial L}{\partial t}(\bm{x}) = C \frac{\sum_{k=1}^{N}b_k\delta(\bm{x}-\bm{x}_k)}{\Delta t},
\end{equation}
where N represents the number of events within $\Delta t$. If events are gathered along the respective warping field, the resultant IWE is a measure of spatial intensity gradient projected onto respective optical flow
\begin{equation}
    \int_{t_0}^{t_1}\nabla I \cdot v dt = -C\times \sum_{k=1}^{N}b_k \delta(\bm{x}-\bm{x}_k')/(t_1-t_0).
\end{equation}

Since image gradient clearly contains structural information, the resultant warped Image of Events Correlation (IEC)
\begin{equation}
    \mathrm{IEC}(\bm{x})=\sum_{k=1}^N b_k\delta(\bm{x-x_k'})/\mathrm{timespan},
\end{equation}
can represent temporal correlation between events, i.e., events which originate from the same structure are close to each other spatially and the intensity value measures how strong the events are correlated to each other. Therefore, we can obtain the events correlation by motion estimation. Also since noisy events and interference from other clusters don't come from that motion, they have low correlation compared to real activity events, and we can filter out them based on that information.

\textbf{Loss Function as Sharpness Measure \quad} The objective function of motion estimation is the sharpness of the IWEs. In \cite{stoffregen2019event} the summation of variance of each IWE is used as loss function. However, variance is a statistical quantity that does not contain any structural information. To better incorporate spatial information into the loss function while suppressing the effect of unstructured noise, we use the weighted mean of windowed variance, where weights are chosen to be the corresponding IEC.

Specifically, given a group of warped events $E_{ref}=\{e_k'=(\bm{x}_k',t_{ref})|k=1,2...N\}$, the IWE is first obtained and local variance is calculated for each pixel with respect to the window size. Then the correlation of the resultant local variance image and the IEC is calculated as a final score for sharpness
\begin{align}
    % IWE_i(\bm{x})&=\sum_{i=1}^{N_e} w_i\times\delta(\bm{x-x_i'})\\
    Var_{ik}&=\frac{1}{|\omega|^2}\sum_{j\in\omega_k} (I_{ij}-\mu_{ik})^2\\
    \mathrm{Sharpness}(I_j)&=\frac{\sum_k Var_{jk}\times|IEC_{jk}|}{\sum_k |IEC_{jk}|},
\end{align}
where $\bm{x_i'}=W(\bm{x_i},t,\bm{\theta})$ is the warped location, $W$ is the warp function, and $\omega$ is the window size. The motion parameter $\bm{\theta}$ is optimized to the one that maximizes the loss function.

As is shown in Fig.\ref{}, the warped image is quite sparse, but by our local variance formulation those areas with no events are discarded and only regions with apparent structure are accounted. It's also worth noting that by weighting with IEC, the fake structures from event noise are also suppressed, promising better motion estimation results.

After obtaining the loss function, the gradient with respect to each motion parameter is calculated, then we can apply some optimization algorithms to maximize it.
\begin{equation}
    \bm{\theta}\gets\bm{\theta}+\mu\nabla_{\bm{\theta}}\textrm{Sharpness},
\end{equation}

If the window size $\omega$ is too small then the calculated local variance cannot capture useful information, but if it's too large some regions with no information are also considered. In practice we choose the window size that maximizes the aggregated local variance, compromising those two factors. Experimental results show our proposed loss function can effectively improve the motion estimation performance.

\textbf{Probability Assignment for Different Clusters\quad} Now we need to output segmentation labels based on the correlation of each event with all the clusters. The output should sum up to 1 in order to represent event assignment probability.

Specifically, contribution of each event to the IWE is calculated as the value of IWE at it's warped location or denoted as local contrast as in \cite{stoffregen2019event}:
\begin{align}
    c_{ij} &= I_j(x_i)\\
    p_{ij} &= \frac{c_{ij}}{\sum_{j=1}^{N_l} c_{ij}}
\end{align}

\subsection{Event Denoising Module}
For a group of $N$ events $E=\{e_i=(x_i,y_i,t_i,k_i)|i=1,2...N\}$, we want to find its segmentation representation as weights in weighted event space $\Omega$ that both has the property of probability but also considers the effect of noise. To do this, besides the normal event probability map as a matrix of shape $N\times N_l$, we calculate individual event confidence to be real as a matrix also of shape $N\times N_l$ representing the confidence for an event to be real in each motion group. This, when multiplied by the event probability map, provides a representation of segmentation result in $\Omega$. In theory, if an event does not belong to some motion groups, then its confidence to be in those groups should also be close to zero, which is implemented intentionally in our method.

The denoising part takes IEC as input, and returns the confidence of each event being real aggressively. "Aggressive" means it tries to give confidence 1 to those events with high contribution and confidence 0 to those with near-zero contribution.

Specifically, we can construct the IEC by building histograms of the warped events weighted by polarity or by some kernel methods, then the event correlation for event $i$ in motion group $j$ can be calculated as the absolute value at warped location:
\begin{equation}
    EC_{ij}&=|IEC_j(\bm{x_i'})|,
\end{equation}
where $timespan$ represents the duration of the event stream as a normalizing factor.

The correlation is then mapped to the range of [0,1] to represent the confidence of that event. Current implementation uses tanh as the mapping function
\begin{equation}
    c_{ij}=tanh(\lambda EC_{ij}),
\end{equation}
where $\lambda$ is the normalizing factor that controls the denoising level. It's worth noting that those events with probability near zero will have high confidence that it is noise, so there is no need to manually exclude those events that do not belong to the cluster under consideration.
%%%

% \subsection{Warped Event Image As Event Correlation Representation}
% The output of DVS, or event stream takes the form of spatio-temporal pointcloud, i.e. $E=\{e_k=(\bm{x}_k,t_k,p_k)|k=1,2...N_e\}$, where each event $e_k$ represents a change in logarithmic intensity at pixel $\bm{x}_k$ and time $t_k$ % 要不要说明下噪声很大
% \begin{equation}
%     \Delta L(\bm{x}_k,t_k)=L(\bm{x}_k,t_k)-L(\bm{x}_k, t_k-\Delta t_k)=p_k C,
% \end{equation}
% where $L(\bm{x},t)=logI(\bm{x},t)$ and $C$ is contrast threshold.
% The fact that only intensity changes are recorded makes it inherently a spares representation of scene illumination, thus a new event correlation metric needs to be developed to extract useful information for subsequent applications like optical flow estimation or motion segmentation.

% % Inspired by pointcloud processing techniques, some early optical flow works utilize spatio-temporal correlation as the correlation metric to filter out noise events, i.e. real events can usually find a new event within its spatio-temporal window
% Inspired by pointcloud processing techniques, some early works\cite{} process each event within its spatio-temporal window. However, the randomly spaced events usually make it hard to determine the size of each spatio-temporal window. Besides, the fact that events represents intensity changes is not well exploited in their approaches. Recently, some works utilize the concept of Image of Warped Events (IWE) from an optimization point of view. Specifically, all events are summed up (possibly by a weight) along a warp field $\bm{W}$ to build an image as
% \begin{equation}
%     I_j(\bm{x})=\sum_{k=1}^{N_e}w_k\delta(\bm{x}-\bm{x}_{k}'),
% \end{equation}
% where $w_k$ is the weight of $e_k$ and $\bm{x}_k'=\bm{W}(\bm{x}_k,t_k;\bm{\theta}_k)$ is the warped event location by a warping parameter $\bm{\theta}_k$
% \begin{equation}
%     e_k=(\bm{x}_k,t_k,p_k)\mapsto e_k'=(\bm{x}_k',t_{ref},p_k).
% \end{equation}
% It's often easier and more robust to optimize in this 2D space than in the full 3D space.

% Based on this observation, we regard the warped image as a 2D representation of events in 3D space, i.e. a dimensionality reduction representation of events cloud, but arbitrarily warped IWE does not contain any usefuly information. Based on the brightness constancy constraint\cite{}, we have
% \begin{equation}
%     \frac{\partial I}{\partial t} = -\nabla I \cdot v,
% \end{equation}
% where $v$ is the velocity in the image space. For DVS, output events can be regarded as a measure of temporal gradient of intensity, thus, if events are gathered along the respective warp field, the resultant IWE is a measure of spatial intensity gradient projected onto respective optical flow
% \begin{equation}
%     \int_{t_0}^{t_1}\nabla I \cdot v dt = -C\times \sum_{k=1}^{N_e}p_k \delta(\bm{x}-\bm{x}_k')/(t_1-t_0),
% \end{equation}
% where $N_e$ is the number of events in $[t_0, t_1)$. This representation clearly represents events correlation, i.e., events which originate from the same structure are close to each other spatially and the intensity value measures how strong the events are correlated to each other. Therefore, we can obtain the events correlation by motion estimation. Also since fake events (noise) don't come from motion, they have low correlation compared to real events, and we can filter out fake events based on that.

% \subsection{Problem Statement}
% For the problem of motion segmentation, we conform with the notation in \cite{stoffregen2019event} in that every event should be assigned a segmentation probability for a finite number of motion groups but take a step further in that probability is replaced by the notation ``weight'' that may represent any value in the range [0,1]. In that way, with $N_l$ possible motion groups, each event has also $N_l$ weights $w_i$ that function like channels in ordinary images. With that in mind, events are processed in weighted event space regardless of the specific value for each channel, and is denoted by $\Omega$.

% For a group of $N$ events $E=\{e_i=(x_i,y_i,t_i,p_i,\bm{w_i})|e_i\in\Omega, i=1,2...N\}\subset\Omega$, we want to find its segmentation representation as weights in weighted event space $\Omega$ that both has the property of probability but also considers the effect of noise. To do this, besides the normal event probability map as a matrix of shape $N\times N_l$, we calculate individual event confidence to be real as a matrix also of shape $N\times N_l$ representing the confidence for an event to be real in each motion group. This, when multiplied by the event probability map, provides a representation of segmentation result in $\Omega$. In theory, if an event does not belong to some motion groups, then its confidence to be in those groups should also be close to zero, which is implemented intentionally in our method. The overview of our proposed method is shown in Fig.\ref{fig:cycle}

% % \subsection{Working Principle of Our Framework}
% % Motion segmentation in the case of event streams means finding out the motion parameter associated with each event point. Since a single event doesn't contain any motion information, this is possible only if a bunch of events is present, just like in the case where optical flow calculation must be done with video instead of a single image. Due to the working principle of event camera, events are mostly triggered along the boundary of objects or texture, thus having a ``tubular'' shape if viewed in x-y-t coordinate as shown on the top part of Fig.\ref{fig:cycle}. So the problem of motion segmentation can also be viewed as finding the respective bounding tube for each event. To do this, one component of motion segmentation called motion estimation is used to predict the future shape of that tube, thus enabling better alignment of events.

% % Our framework is based on the setup of \cite{stoffregen2019event}, where weighted events in x-y-t space are mapped onto the x-y space (image plane) based on the respective motion parameter to produce sharp warped images (IWEs) and probability assignment is calculated based on their contribution to the sharpness. But instead of returning to the warping process directly, we calculate the confidence of each event being real by warping the events additionally weighted by polarity to produce an estimation of Image of Projected Gradient (IPG) and then measure the power of each event.

% % We note that one pixel value of IPG is dependent both on the number of events that lie in it and on their weights and polarities. Thus regions with frequent but irregular positive and negative events will also be filtered out, as is the case of darker areas. But with IWEs only, these regions cannot be ignored and thus affecting the performance of motion segmentation.

% % As is shown in Fig.\ref{fig:cycle}, our progressive motion segmentation framework consists of three parts: the motion segmentation part, the motion estimation part, and the denoising part. The name ``progressive'' comes from the fact that they work in a mutually reinforced manner.

% \subsection{Working Principle of Our Framework}
% As is shown in Fig.\ref{fig:cycle}, our progressive motion segmentation framework consists of three parts: the motion segmentation part, the motion estimation part, and the denoising part. The name ``progressive'' comes from the fact that they work in a mutually reinforced manner.

% The ME module tries to separate the events into different clusters based on their motion information. This is done by a warping process to find the sharpest projected image. Since events are mostly triggered along texture boundaries, this process produces edge-like images representing motion sources. For $N_l$ possible warps, a total of $N_l$ images of warped events (IWEs) are estimated and the significance of each event in those warps can be calculated, which is used to for event clustering. To achieve this, motions must be estimated correctly so interference from other clusters and noise must be suppressed. In the implementation of \cite{stoffregen2019event}, this is done based on the loss function as variance alone.  In our implementation a specially designed Event Denoising (ED) module is used for that purpose.

% The ED module can suppress the effect of noise and interference from other clusters by utilizing the events correlation information estimated from the motion parameter. A coarse motion parameter can still provide some metric for event correlation, making the progressive framework feasible.

% \subsection{Implementation Details}
% \textbf{Denoising Part\quad} The denoising part takes events with estimated motion parameters as input, calculates the images of events correlation (IEC), and returns the confidence of each event being real aggressively. "Aggressive" means it tries to give confidence 1 to those events with high contribution and confidence 0 to those with near-zero contribution.

% Specifically, we can construct the IEC by building histograms of the warped events weighted by polarity or by some kernel methods, then the event correlation for event $i$ in motion group $j$ can be calculated as the absolute value at warped location:
% \begin{align}
%     IEC(\bm{x})&=\sum_{i=1}^N w_i\times p_i \times \delta(\bm{x-x_i'})/timespan\\
%     EC_{ij}&=|IEC_j(\bm{x_i'})|,
% \end{align}
% where $timespan$ represents the duration of the event stream as a normalizing factor.

% The correlation is then mapped to the range of [0,1] to represent the confidence of that event. Current implementation uses tanh as the mapping function
% \begin{equation}
%     conf_{ij}=tanh(\lambda EC_{ij}),
% \end{equation}
% where $\lambda$ is the normalizing factor that controls the denoising level. It's worth noting that those events with probability near zero will have high confidence that it is noise, so there is no need to manually exclude those events that do not belong to the cluster under consideration.

% \textbf{Loss Function of Motion Estimation\quad} The objective function of motion estimation is the sharpness of the IWEs. In \cite{stoffregen2019event} the summation of variance of each IWE is used as loss function. However, variance is a statistical quantity that does not contain any structural information. To better incorporate spatial information into the loss function while suppressing the effect of unstructured noise, we use the weighted mean of windowed variance, where weights are chosen to be the corresponding IEC.

% Specifically, given a group of warped events $E_{ref}$, the IWE is first obtained and local variance is calculated for each pixel based on the window size. Then the correlation of the resultant local variance image and the IEC is calculated as a final score for sharpness

% \begin{align}
%     IWE_i(\bm{x})&=\sum_{i=1}^{N_e} w_i\times\delta(\bm{x-x_i'})\\
%     Var_{ik}&=\frac{1}{|\omega|^2}\sum_{j\in\omega_k} (IWE_{ij}-\mu_{ik})^2\\
%     loss&=\sum_{i=1}^{N_l}\frac{\sum_k Var_{ik}\times|IEC_{ik}|}{\sum_i |IEC_{ik}|},
% \end{align}
% where $\bm{x_i'}=W(\bm{x_i},t,\bm{\theta})$ is the warped location, $W$ is the warp function, and $\omega$ is the window size. The motion parameter $\bm{\theta}$ is optimized to the one that maximizes the loss function.

% As is shown in Fig.\ref{}, the warped image is quite sparse, but by our local variance formulation those areas with no events are discarded and only regions with apparent structure are accounted. It's also worth noting that by weighting with IEC, the fake structures from event noise are also suppressed, promising better motion estimation results.

% After obtaining the loss function, the gradient with respect to each motion parameter is calculated, then we can apply some optimization algorithms to maximize it.
% \begin{equation}
%     \bm{\theta}\gets\bm{\theta}+\mu\nabla_{\bm{\theta}}loss,
% \end{equation}

% If the window size $\omega$ is too small then the calculated local variance cannot capture useful information, but if it's too large some regions with no information are also considered. In practice we choose the window size that maximizes the aggregated local variance, compromising those two factors. Experimental results show our proposed loss function can effectively improve the motion estimation performance.
% % The motion parameter $\bm{\theta}$ is optimized to the one that maximizes the contrast of IWE. We observe that if the kernel function takes a certain form, variance can be calculated analytically. With gaussian kernel with standard deviation $\sigma$, it can be shown that variance can be calculated as:
% % \begin{equation}
% %     Var(IWE(\bm{x}))=\frac{1}{2}\sum_{i,j=1}^N w_i w_j e^{-\frac{r_{ij}^2}{4\sigma^2}}-(\sum_{i=1}^N w_i)^2
% % \end{equation}
% % where $r_{ij}=||\bm{x_i-x_j}||_2$. Thus we don't need to manually specify the reference time and spatial discretization scheme.

% \textbf{Probability Assignment for Different Clusters\quad} Now we need to output segmentation labels based on the correlation of each event with all the clusters. The output should sum up to 1 in order to represent event assignment probability.

% Specifically, contribution of each event to the IWE is calculated as the value of IWE at it's warped location or denoted as local contrast as in \cite{stoffregen2019event}:
% \begin{align}
%     contrib_{ij} &= IWE_j(x_i)\\
%     prob_{ij} &= \frac{contrib_{ij}}{\sum_{j=1}^{N_l} contrib_{ij}}
% \end{align}

% % But it also means that if the MS module fails, the Denoise Module will fail too.

% \textbf{Collaborative Optimization\quad}
% The optimization process quite resembles the one used in EM algorithm, but here we have three parts instead of two. So while optimizing one part, we must fix the other two parts. The pseudocode is shown in Algo.\ref{algo:loop}.
% % The reason to take polarity into account is to help construct the mapping function. Because the number of events in one event packet is uncertain, the central point of that function should shift accordingly, which is hard to determine. It's worth noting that those events with probablity near to zero will have a high confidence that it is noise, so there is no need to manually exclude those events that do not belong to the cluster under consideration. But it also means that if the MS module fails, the Denoise module will fail too.

% % In the cycle of the above three modules, only weights get updated, i.e. the input to the Denoise module is the input to the MS module weighted by probablity, and the input to the CM module is the input to the Denoise module weighted by confidence. The pseudocode is shown below:

% \begin{algorithm}
% \SetAlgoLined

% \KwResult{Probablity Assignment Prob, Event Confidence Conf, Motion Parameter $\bm{\theta}$}
%  Prob=1/NumMotions,Conf=1,W=1\;
%  \While{Denoise Diverging}{
%   \While{MS Diverging}{
%      \While{CM Diverging}{
%       \ForEach{motion in $\bm{\theta}$}{
%          $E_{ref}$ = warp($E$,motion)\;
%          IWE = KDE(gImg)\;
%          motion = $\underset{motion}{\arg\max}$ Var(IWE)\;
%       }
%      }
%      $c_{ij} = pImg_j(x_i)$\;
%      $Prob_{ij} = \frac{c_{ij}}{\sum_{j=1}^l c_{ij}}$\;
%      $W=W\times Prob$\;
%   }
%   $IPG=\operatorname{KDE}(gImg\times polarity)$\;
%   $cp_{ij}=IPG_j(x_i)$\;
%   $Conf=tanh(\lambda|cp_{ij}|)$\;
%   $W=W*Conf$
%  }
%  \caption{Progressive Motion Segmentation By Gradient Image Denoising\label{algo:loop}}
% \end{algorithm}
